Deformable Graph Transformer

Transformer-based models have recently shown success in representation learning on graph-structured data beyond natural language processing and computer vision. However, the success is limited to small-scale graphs due to the drawbacks of full dot-product attention on graphs such as the quadratic complexity with respect to the number of nodes and message aggregation from enormous irrelevant nodes. To address these issues, we propose Deformable Graph Transformer (DGT) that performs sparse attention via dynamically sampled relevant nodes for efficiently handling large-scale graphs with a linear complexity in the number of nodes. Specifically, our framework first constructs multiple node sequences with various criteria to consider both structural and semantic proximity. Then, combining with our learnable Katz Positional Encodings, the sparse attention is applied to the node sequences for learning node representations with a significantly reduced computational cost. Extensive experiments demonstrate that our DGT achieves state-of-the-art performance on 7 graph benchmark datasets with 2.5 - 449 times less computational cost compared to transformer-based graph models with full attention.

==> 2_related_works/2_0_related_works_bak.tex <==
\label{sec:related_works}
\paragraph{Attention based methods for graphs.}
Attention mechanisms have become the \textit{de facto} necessity, allowing the model to focus on the relevant parts of the input for the target task \citep{attention1, attention2}. Motivated by the success of the attention mechanisms, there have been many works that apply them to graph neural networks \citep{graphattention2, GAT,GATv2,superGAT,gtn,HGT,HAN}.
% attention mechanism has been adopted to allocate larger weights to important neighbor nodes []. 
% GAT~\citep{GAT} compute the representation of each node by attending over its neighbors, leveraging self-attentional layers. 
GAT~\citep{GAT} adaptively aggregates messages from neighborhoods with the attention scheme.
\citep{GATv2} proposes a more expressive graph attention network named GATv2 by simply modifying the attention operation of GAT. 
% \citep{superGAT} suggests a self-supervised learning scheme of learning attention to distinguish relevant information from messages of all neighbors. 
% \citep{gtn} uses attention scores for different edge types to represent a weighted sum of meta-paths.
% //TODO: GTN 한줄 설명

Recently, \citep{Graphomer,GT,GraphiT,SAN,GraphTrans} have directly adopted the Transformer architecture for learning on graphs. 
Graphormer~\citep{Graphomer} and GT~\citep{GT} are built upon the standard Transformer architectures by incorporating structural information of graphs into the attention.
\citep{GraphBert} also utilizes the graph-specific positional features to capture absolute and relative node positional information.
% \citep{HGT} 
However, these approaches 
% are limited to graph-level prediction, where the target graphs consist of a small number of nodes and 
are not suitable for node-level prediction with large-scale graphs. 
It is because referencing numerous key nodes for each query node is prohibitively costly and that might hinder the attention function from learning the proper weights for each key node.
Although restricting the attention scope to k-hop local neighbors \citep{GT} might reduce the computational complexity, it causes a limited receptive field.
To mitigate the issues of existing graph Transformers, our DGT dynamically samples the key/value pairs to achieve sparse attention.
% causes the loss of global information which is the main advantage of Transformer architecture.
% \textcolor{red}{Ours}

\paragraph{Transformer based methods.}
% The Transformer \citep{Transformer} and its variants \citep{Bert,GPT3,sparseTransformer} have proven beneficial for capturing global dependencies between input and output and have been widely used for natural language processing. 
% It also attains excellent results in image recognition by directly applying its architecture to the sequences of image patches \citep{ViT, Swintransformer, Focal, DETR, DeformableDETR}.
The Transformer~\citep{Transformer} and its variants have achieved performance improvements in various domains such as natural language processing~\citep{Bert,GPT3} and computer vision~\citep{ViT,DETR,Swintransformer}. 
However, training these models needs quadratic space and time complexity, which is especially problematic with long input sequences.
Recent works~\citep{Performer,Perceiver,patternattention1,patternattention2,Reformer} have studied this issue and proposed various efficient Transformer architectures.
\citep{Performer, Nystromformer,lowrankattention1} study the low-rank approximation for attention to reduce the complexity.
Perceiver~\citep{Perceiver, PerceiverIO} leverages a cross-attention mechanism to recursively distill inputs into latent vectors to scale linearly with the size of inputs.  
% The model scales linearly with the size of inputs and outputs by having the fixed size of the latent array as keys.
Sparse Transformer~\citep{sparseTransformer} uses pre-defined sparse attention patterns on keys by restricting the attention pattern to be fixed local windows.
\citep{DeformableDETR} also proposes sparse attention that dynamically samples a set of key/value pairs for each query without a fixed attention pattern.
Inspired by the deformable attention~\citep{DeformableDETR,DAT}, we propose deformable attention for graph-structured data that flexibly attends to informative key nodes considering various types of the proximity between nodes.
% \textcolor{red}{Ours}. 

% \newpage
% However, generalizing the deformable attention mechanism on graph-structured data has two main challenges.
% Unlike image recognition which has continuous pixel values, nodes in graphs are in a discrete space.
% Thus, just focusing on a small fixed set of sampled points might not be sufficient for the offsets to move to the fairly relevant data point. 
% To address this issue, we adopt the Radial Basis Function kernel to look up at a wide range of nodes.
% In addition, computing offsets of the key nodes for the query node is challenging due to the non-Euclidean nature of graph-structured data. 
% We first define the direction and the distance among nodes with various aspects, such as BFS, PPR, and feature similarity, and use these pre-defined sets of node sequences to learn the offsets for the key-value pairs.

% graph representation learning
% efficient transformers
% \paragraph{Graph Neural Networks.}
% \begin{itemize}
%     \item Overall graph neural network
%     \item GNNs for heterophily~(Geom-GCN~\citep{Geom-GCN}, H2GCN~\citep{H2GCN}, GPRGNN~\citep{GPRGNN}, DeformableGCN)
% \end{itemize}
% \paragraph{Graph Attention Mechanisms.}
% \begin{itemize}
%     \item existing attention based graph neural networks,   (GAT~\citep{GAT}, GATv2~\citep{GATv2}, SuperGAT)
%     \item Graph Transformer
% \end{itemize}
% \paragraph{Transformer based Methods.}
% \begin{itemize}
%     \item Transformer - nlp, computer vision~(Transformer~\citep{Transformer}, ViT~\citep{ViT}, Swin Transformer~\citep{Swintransformer}, DETR~\citep{DETR}
%     \item Efficient Transformer 
%     \begin{itemize}
%         \item Attention with compressed sequences (e.g., Perceiver~\citep{Perceiver}, PerceiverIO~\citep{PerceiverIO})
%         \item Low-rank/kernel-based methods relying on the decomposition of the attention matrix (e.g., Performer~\citep{Performer}, Nystromformer~\citep{Nystromformer})
%         \item Sparsifying attention (e.g., Reformer~\citep{Reformer}, sparse Transformer~\citep{sparseTransformer}, Deformable DETR~\citep{DeformableDETR})
%     \end{itemize}

%     reformer, performer, perceiver, deformable detr, sparse Trnsformer
% \end{itemize}


==> 3_methods/3_1_preliminaries_bak.tex <==
\paragraph{Graph Neural Networks (GNNs).} 
Consider an undirected graph $\mathcal{G}=(\mathcal{V},\mathcal{E})$ with a set of $N$ nodes $\mathcal{V} = \{v_1, v_2, \dots, v_N\}$ and a set of edges $\mathcal{E} = \{ (v_i, v_j)\ \vert\ v_i, v_j \in \mathcal{V} \}$ where the nodes $v_i, v_j \in \mathcal{V}$ are connected. 
Each node $v_i \in \mathcal{V}$ has a feature vector $\xb_{i} \in \Rbb^{F}$, where $F$ is the dimensionality of the node feature, and a set of neighborhoods $\mathcal{N}{(i)}=\{v_j \in \mathcal{V}|(v_i,v_j) \in \mathcal{E}\}$. 

Given a graph $\mathcal{G}$ and a set of node features $\left\{\xb_i\right\}_{i=1}^{N}$, Graph Neural Networks (GNNs) aim to learn each node representation by an iterative aggregation of transformed representations of the node itself and its neighborhoods as follows:
\begin{equation}
{\textbf{h}}^{(l)}_i = \sigma \left ( \textbf{W}^{(l)}\left ( c_{ii}^{(l)}\textbf{h}_i^{(l-1)} + \sum_{v_j \in \mathcal{N}{(i)}}{c_{ij}^{(l)}\textbf{h}_j^{(l-1)}}\right )   \right ), 
\label{eq:gnn}
\end{equation}
% \begin{equation}
% {\textbf{h}}^{(l)}_v = \sigma \left ( \sum_{u \in \Tilde{\mathcal{N}}_v}{c_{uv}^{(l)}\textbf{W}^{(l)}\textbf{h}_u^{(l-1)}}\right ) , 
% \label{eq:gnn}
% \end{equation}
% \begin{equation}
% {h}^{(l)}_v = \sigma \left ( W^{(l)}\left ( c_{vv}^{(l)}h_v^{(l-1)} + \sum_{u \in \mathcal{N}_v}{c_{uv}^{(l)}h_u^{(l-1)}}\right )   \right ), 
% \label{eq:gnn}
% \end{equation}
where ${\hb}^{(l)}_i \in \Rbb^{d^{(l)}}$ is a hidden representation of node $v_i$ in the $l$-th GNN layer,  ${\hb}^{(0)}_i=\xb_i$, $\Wb^{(l)} \in \Rbb^{d^{(l)} \times d^{(l-1)}}$ is a learnable weight matrix at the $l$-th GNN layer, $\sigma$ is a non-linear activation function, $c_{ij}^{(l)}$ and $c_{ii}^{(l)}$ represent weights for aggregation characterized by each GNN. 
For example, GCN  \citep{GCN} can be represented as a form of (\ref{eq:gnn}) if $c_{ij} = (\text{deg}(i)\text{deg}(j))^{-1/2}$ and $c_{ii} = (\text{deg}(i))^{-1}$, where $\text{deg}(i)$ is the degree of node $v_i$, and GAT \citep{GAT} learns $c_{ij}^{(l)}$ and $c_{ii}^{(l)}$ based on the attention mechanism.

\paragraph{Attention in Transformer.}
Transformers~\citep{Transformer} have shown their superior performance based on multi-head self attention mechanisms.
% Given a query vector $\zb_q \in \Rbb^c$ and set of key vectors $\Fc = \left\{\fb_k \right\}_{k \in \Omega_k}$, where $q \in \Omega_q$ is an index of the query and $\Omega_q, \Omega_k$ are the set of query and key indices, the multi-head attention~(MHAttn) is formulated as follows:
Given a query index $q \in \Omega_q$ with a corresponding vector $\zb_q \in \Rbb^c$ and a set of key/value vectors $\Fc = \left\{\fb_k \right\}_{k \in \Omega_k}$, where $\Omega_q, \Omega_k$ are the set of query and key indices, the Multi-Head Attention~(MHA) is formulated as follows:
\begin{equation}
\label{eq:mhattn}
    \text{MHA}\left(\zb_q, \Fc\right) = \sum_{m=1}^M \Wb_m \left[\sum_{k \in \Omega_k} \Ab_{mqk} \cdot \Wb^\prime_m \fb_k \right],
\end{equation}
where $m$ is the index of $M$ attention heads, $\Wb_m \in \Rbb^{c \times c_v}$ and $\Wb_m^\prime \in \Rbb^{c_v \times c}$ are weight matrix parameters. 
The attention weight $\Ab_{mqk}$ between the query $\mathbf{z}_q \in \Rbb^c$ and the key $\fb_k \in \Rbb^c$, which is generally calculated as $\Ab_{mqk} = \frac{\exp\left[{\zb_q^\top \Ub^\top_m \Vb_m \fb_k}/{\sqrt{c_v}} \right]}{Z}$, where $Z \in \mathbb{R}$ is a normalization factor to achieve $\sum_{k\in \Omega_k} \Ab_{mqk}=1$ and $\Ub_m, \Vb_m$ are weight matrices to compute queries and keys, respectively. 
% The known issue of the multi-head attention is a high computational complexity.
Although the multi-head attention operation contributes to the success of the Transformer-based models, it has a known issue of substantial computational costs and large memory.

% \textcolor{blue}{The scalability issue has been extensively studied in the literature.}
This scalability issue has been extensively studied in the literature. 
However, most efficient attention methods have been developed by either limiting the attention within a local neighborhood or approximating an attention map with a low-rank matrix.
The former approaches are problematic when neighbors belong to different classes as heterophilic graphs, and the latter approaches tend to yield \textit{dense} attention leading to enormous messages from irrelevant nodes. 
So, we adopt a more flexible and efficient Deformable Attention ~\citep{DeformableDETR,DAT} that performs a \textit{sparse} attention by dynamically sampling a small set of relevant keys without a predefined window.
% \sjy{This scalability issue has been extensively studied in the literature.While most efficient attention methods addressed the issue by limiting the attention computation within a \textit{fixed} local range or approximating the \textit{entire} attention matrix with a low-rank matrix, deformable attention ~\citep{DeformableDETR,DAT} performs a sparse attention by flexibly sampling a small set of relevant keys without a predefined and fixed range.}
% However, most efficient attention belong to either limited attention within small neighborhoods or efficient computation of global attention map. 
% To reduce the computational cost with preserving the advantage of Transformer that captures long-range dependencies, deformable attention has been proposed.
% 
% 
% Deformable
% \textcolor{blue}{In computer vision, one of the methods to address the above issue is a deformable attention module~\citep{DeformableDETR,DAT}. 
% \sjy{(Deformable attention is a data-dependent sparse attention that samples relevant keys for each query by predicting coordinates of them on the input feature map and performs attention with sampled keys.)}
Let $\fb \in \Rbb^{c \times h \times w}$ be an input feature map and $\pb_q$ be a position of query $\zb_q$.
Then, the DeFormable Attention~(DFA) is defined as
% \paragraph{Deformable Attention~\citep{DeformableDETR}.}
\begin{equation}
    \text{DFA}\left(\zb_q, \pb_q, \Fc \right) = \sum_{m=1}^M \Wb_m\left[\sum_{k=1}^K\Ab_{mqk}\cdot \Wb^\prime_m \fb\left(\pb_q + \Delta \pb_{mqk} \right) \right],
\end{equation}
where $k$ is an index of sampled key vectors, and $K$ is the total number of the key.  
The attention weight $\Ab_{mqk}$ of $m$-th attention head has a value between 0 and 1, normalized by $\sum_{k=1}^K \Ab_{mqk}=1$ similar to the multi-head attention.
$\Delta \pb_{mqk} = \Wb_{mk} \zb_q$ is a sampling offset of the $k$-th sampling key of the $m$-th attention head.
Since the deformable attention module uses only a small set of informative keys for each query, it has linear complexity in the number of inputs.
% By reducing the number of key nodes, it is possible to make transformer-based architecture effective and efficient on large-scale graphs. 

% complexity discussion

% \textcolor{blue}{As stated in Section.~\ref{sec:related_works}, several methods~\citep{Graphomer,GT} have been proposed to harness the power of the standard multi-head attention on graph-structured data.
% Although they have shown superior performance on various graph-related tasks, they have difficulty in learning representations on large-scale graphs.
% Since the large-scale graph has a vast number of nodes, the scalability issue of the multi-head attention is dramatically magnified.
% Also, the enormous number of keys to attend per query node leads to the risk of the aggregation of noisy information from irrelevant key nodes. 
% In this paper, we design an attention module that attends to only a small number of relevant keys different from standard attention that blindly aggregates irrelevant key nodes.}

% several methods
In recent, Transformer-based models~\citep{Graphomer,GT} have been proposed to harness the power of the standard multi-head attention for representing nodes in graphs.
Although they have shown superior performance on various tasks, they have difficulty in learning representations on large-scale graphs.
Since the large-scale graph has a vast number of nodes, the scalability issue of the multi-head attention is dramatically exacerbated.
Also, the enormous number of keys to attend per query node increases the risk of the aggregation of noisy information from irrelevant key nodes. 
In this paper, we design a sparse attention module, Deformable Graph Attention, that attends to only a small number of relevant keys different from standard attention that blindly aggregates irrelevant key nodes.
By reducing the number of key nodes, it is possible to make transformer-based architecture effective and efficient on large-scale graphs. 
% In this paper, summarize the strong points of our paper compared to other transformer-based models
% Node classification ??
% scalability (excessive attention computation)
% excessive number of key -> computational cost, risk of overfitting
% positional encoding

% transformer complexity issue -> in vision deformable attention -> graph domain transformer has a similar issue -> architecture적으로 바꾸려는 시도조차 없다는 것도 강조

==> Checklist/checklist.tex <==
\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~2.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See the Section~\ref{sec:1}.}
  \item Did you describe the limitations of your work?
    \answerYes{See the supplement.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See the supplement.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See the supplement.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See the supplement.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See the Section~\ref{sec:4}.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See the supplement.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See the supplement.}
  \item Did you mention the license of the assets?
    \answerYes{See the supplement.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See the supplement.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{See the supplement.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See the supplement.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Figure_tex/kernel.tex <==
\begin{figure}[t]
\centering
\subfigure[Actor]{
\label{subfig:actor}
\includegraphics[width=0.48\textwidth]{Figures/actor_bandwidth_v7.pdf}
}
% \hspace{0.7cm}
\subfigure[Cora]{
\includegraphics[width=0.48\textwidth]{Figures/cora_bandwidth_v7.pdf}
}
% \subfigure[Pubmed]{
% \includegraphics[width=0.30\textwidth]{Figures/abblation_temp2.png}
% }
\caption{Analysis of our kernel-based interpolation with various bandwidths,  $\gamma = 1,2,4,8,16$.
}
\label{fig:interpolation}
\end{figure}

==> Tables/dataset.tex <==
\begin{table}[t]
  \caption{Dataset statistics.}
  \centering
  \setlength{\tabcolsep}{-1.5pt}
%   \begin{adjustbox}{width=1.0\textwidth}
% ogbn-arxiv &(twitch-gamers)
  \resizebox{\textwidth}{!}{\begin{tabular}{C{1.8cm}C{1.7cm}C{1.7cm}C{1.7cm}C{1.7cm}C{1.7cm}C{1.7cm}C{1.7cm}C{1.7cm}C{1.7cm}}
    \toprule
    Dataset        &   Actor & Squirrel & {Chameleon} &{twitch-gamers} & {Cora} & {Citeseer} & {Pubmed}  & {ogbn-arxiv} & {Reddit} \\
    % \midrule
    \midrule
    \# Classes     &       5 &       5 &      5 &       2&    7 &     6 &     3 &      40 &  41 \\
    \# Nodes       &    7,600 &    5,201 &   2,277 &  168,114& 2,708 &  3,327 & 19,717 &  169,343 & 232,965  \\ 
    \# Edges       &   26,659 &  198,353 &  31,371 & 6,797,557& 5,278 & 4,552 & 44,324 & 1,166,243 & 11,606,919 \\
    Avg degree     &    7.02 &   76.28 &  27.55 &   80.87& 3.90 &  3.03 &  4.50 &   13.67 & 49.82 \\ 
    \bottomrule
  \end{tabular}}
  \label{tab:data_statistics}
%   \end{adjustbox}
\end{table}

% \begin{table}[ht]
%   \caption{Dataset statistics.}
%   \centering
% %   \footnotesize
% %   \setlength{\tabcolsep}{-1pt}
% %   \begin{adjustbox}{width=1.0\textwidth}
% % ogbn-arxiv &(twitch-gamers)
%   \resizebox{\textwidth}{!}{\begin{tabular}{ccccccccc}
%     \toprule
%     Dataset        &   \textbf{Actor} & \textbf{Squirrel} & \textbf{Chameleon} & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Cora} & \textbf{ogbn-arxiv} &\textbf{twitch-gamers} \\
%     % \midrule
%     \midrule
%     \# Classes     &       5 &       5 &      5 &     6 &     3 &    7 &      40 &       2 \\
%     \# Nodes       &    7600 &    5201 &   2277 &  3327 & 19717 & 2708 &  169343 &  168114 \\ 
%     \# Edges       &   26659 &  198353 &  31371 &  4552 & 44324 & 5278 & 1166243 & 6797557 \\
%     \# Features    &     932 &    2089 &   2325 &  3703 &   500 & 1433 &     128 &       7 \\
%     Avg degree     &    7.02 &   76.28 &  27.55 &  3.03 &  4.50 & 3.90 &   13.67 &   80.87 \\ 
%     Hom. ratio $h$ &    0.22 &    0.22 &   0.23 &  0.74 &  0.80 & 0.81 &      -- &      -- \\
%     \bottomrule
%   \end{tabular}}
%   \label{tab:data_statistics}
% %   \end{adjustbox}
% \end{table}
% & arxiv &twitch
% &      40 &       2
% &  169343 &  168114
% & 1166243 & 6797557 
% &     128 &       7 
% &   13.67 &      -- 
% &      -- &      -- 
